Towards Efficient Integration of Blockchain for IoT Security: The Case Study of IoT Remote Access

The booming Internet of Things (IoT) market has drawn tremendous interest from cyber attackers. The centralized cloud-based IoT service architecture has serious limitations in terms of security, availability, and scalability, and is subject to single points of failure (SPOF). Recently, accommodating IoT services on blockchains has become a trend for better security, privacy, and reliability. However, blockchain's shortcomings of high cost, low throughput, and long latency make it unsuitable for IoT applications. In this paper, we take a retrospection of existing blockchain-based IoT solutions and propose a framework for efficient blockchain and IoT integration. Following the framework, we design a novel blockchain-assisted decentralized IoT remote accessing system, RS-IoT, which has the advantage of defending IoT devices against zero-day attacks without relying on any trusted third-party. By introducing incentives and penalties enforced by smart contracts, our work enables "an economic approach" to thwarting the majority of attackers who aim to achieve monetary gains. Our work presents an example of how blockchain can be used to ensure the fairness of service trading in a decentralized environment and punish misbehaviors objectively. We show the security of RS-IoT via detailed security analyses. Finally, we demonstrate its scalability, efficiency, and usability through a proof-of-concept implementation on the Ethereum testnet blockchain.

==> sections/cloudassited.tex <==
\section{System Model \& Problem Statement}\label{sec:cur}
\subsection{Relay-assisted IoT Remote Accessing Model}




\subsection{Problems \& Challenges}


\subsection{Threat Model}



==> sections/introduction.tex <==
\section{Introduction}
The IoT market is flourishing. The number of connected things has surpassed 
the global population in 2017 and is estimated to reach 20 billion in 2020~\cite{20b}. IoT devices such as IP cameras and smart light bulbs have been deployed in numerous smart environments. However, different from traditional computing platforms like PCs and Smartphones, IoT devices typically lack
computational resources for enforcing strong security mechanisms. Worse, 
a lot of manufacturers mainly concentrate on novel features, while security flaws  of their things
are left unpatched for years \cite{dlinknopatch}. Consequently, massive vulnerable IoT devices 
are taken down by botnet attackers for large-scale botnet attacks. The astonishing 
damage of IoT botnet attacks was demonstrated by the Mirai attack \cite{Antonakakis2017} in 
September 2016, when more than 600k IoT devices were infected to launch the 
record-breaking DDoS attack. 

Such IP-scanning based harvesting attacks mainly target things that have
public IP addresses; thus, things behind Network Address Translation (NAT)
are protected from such attacks. On the other hand, things isolated by NAT
typically connect to their vendor-maintained (or sponsored) clouds, such that
messages between things and users' control devices can be relayed
by the connected cloud servers and data can be stored in clouds. 
Such a centralized remote-accessing model for things, however, has multiple serious limitations
in terms of security, availability and scalability. 

First, the security of these cloud computing platforms is questionable. 
Major cloud security breaches have been reported for many times~\cite{cloud-breach},
%https://blog.storagecraft.com/7-infamous-cloud-security-breaches/
which shows that even major cloud computing providers such as Amazon cannot
avoid them, let alone the small clouds maintained or sponsored by vendors of those low-cost
IoT devices. As we will describe in section \ref{sec:cur}, 
a lot of such cloud servers run without sufficient security measures. 
Since attacks targeting IoT devices have become
increasingly sophisticated, attackers are certainly motivated to
compromise these cloud servers, which have access privileges to
things that are otherwise protected by NAT, in order to harvest things. 
Once a cloud server in the centralized model is compromised.
a large number of things behind NAT are exposed to attackers.
%Such an attack vector has been employed in practice~\cite{xyz} (\todo{Chenglong, citation please}).
Second, the centralized accessing model is subject to single
points of failure. If a cloud is down, it is unknown how 
the things that are registered (usually, hardcoded in firmware) to use
the cloud can be accessed. Third, the centralized model may not
be scalable enough to meet the requirement of the rapidly
developed market and handle spikes of user requests. 

%Fortunately, home routers' Network Address Translation (NAT) protects the vulnerable devices behind it by blocking direct IP scanning from the Internet. However, isolation of NAT also introduce the problem of device remote access outside the home network. Current home IoT solutions usually choose to add relay modules on the vendor maintained IoT backend cloud server with publicly accessible IP address to relay packets between user's control devices and IoT devices. For the purpose, IoT devices are shipped with hard-coded domain name or IP address of the relay cloud in their firmware for proactive connection after device booting.


%The cloud server which  has a publicly accessible domain name or IP functions as an IoT accessing platform. Thus, the task of NAT traversal for remote access is solved by hardcoding the relay server's IP or domain name into IoT devices and letting them proactively initiate connections towards the relay server.



%IoT botnet malwares use the same scanning method as other botnet malware by randomly generating IP addresses for scanning. Fortunately, home routers' Network Address Translation (NAT) serves as an effective shield to block these inward scanning traffic. 

% as an aggregated accessing platform for all connected products from the vendor. The NAT traversal problem is solved by hardcoding the cloud server's domain name into IoT devices' firmware to let them launch proactive heartbeat connection with the cloud server on powered up. 


% disabling all inward traffic and isolating the IoT devices in the private network behind the NAT also impose impediment for user's remote access. Under this case, users need to stay in the same private network with the IoT devices for direct access.



% As a result, IoT devices with public IP would bear the first brunt of malware infection while other consumer IoT devices which are behind the home router's Network Address Translation (NAT) can keep free of these malicious scanning. This also explains why home routers become a primary target in following waves IoT malware attack after Mirai and a lot of security

% guidelines\cite{diableportmapping,xfinitysecurity,internetkeepsafe} for home IoT device recommend disabling all port mapping on home routers to avoid exposing device to public Internet.



%Though solves the NAT traverse problem, centralized relay server, in turn, may become attractive targets for botnet attackers. To reduce the traffic and cost, as we will present in section \ref{sec:cur}, a lot of cloud servers are operating without sufficient security implementation, especially for some low-cost IoT device vendors who outsource cloud service for their products to third-party service providers. As a result, these vulnerable relay clouds assist attackers by aggregating access to a mass of IoT devices \emph{that are originally protected by NAT} which helps them perform more accurate and efficient victim searching. 
%From the perspective of attackers, they can get direct access to all connected devices once they can take down or cheating the centralized relay server, in which way they can proceed to infect these IoT devices without conducting the time-consuming random scanning. 
%Moreover, IoT's model name and software details may also be leaked to attackers for more accurate malware development.

% If cloud relay server is taken down by cyber attacks, attackers can then utilize the server to deliver malicious packets to all connected devices in short time, device's model name and software details may also be exploited for launching more accurate attacks.

% Unfortunately, as we'll illustrate in section\ref{sec:vul_in_cloud}, a lot of IoT devices are operated on vulnerable cloud services. Some low-cost device vendors' cloud servers relay packets to connected IoT devices without authenticating sender's identity. There is no surprise because security implementation is not only costly but isn't that appealing as other fancy functions. 

Some solutions are proposed to defeat IoT malware like Mirai. They 
employ malware detection or honeypots~\cite{luo2017iotcandyjar,thakar2017reverse} to 
passively collect malware's characteristics for discovering and taking down the botnet 
master node. These method cannot provide comprehensive and timely protection. 
Other defense methods are either not flexible or require strong security assumptions; 
e.g., assuming that IoT devices are built on hardware with specific security features \cite{winter2008trusted,costan2016intel}.



\paragraph{This Work}
In this paper, we propose \textsc{RS-IoT}, a novel IoT remote accessing solution based on decentralized relay sharing. The intrinsic advantage of the decentralized architecture provides a robust solution to aforementioned problems in security, availability, and scalability. Leveraging the power of smart contracts, we design a transparent, self-governing relay service trading platform  where \emph{monetary incentives} are used to motivate third-party relay service providers' participation and deter potential malicious behaviors.  By enforcing monetary penalties, the proposed technique
is able to thwart attackers who aim at making profits from attacks. More remarkable, the reporting and proof-of-delivery mechanism is able to tackle the zero-day attacks, and solve disputation of cheating without the need of any trusted authorities. People have realized that cyber security is not a problem that only technology can solve and 
tried to include also an economic point of view~\cite{jerman2008economic}, while
we have effectively enabled ``\emph{an economic approach to cyber security}''~\cite{economic} when resolving this important 
security problem. 

This paper focuses on the security aspect when presenting the system. As we will show, 
since security is enforced by the proposed technique, IoT devices owners on this platform can freely 
commission arbitrary relay service providers instead of the ones specified by vendors. Thus,
the decentralized nature of the proposed technique naturally resolves the availability and  scalability 
issues of the current centralized model. 

\paragraph{Contribution}
Our main contributions are as follows:
\begin{itemize}
	\item To the best of our knowledge, RS-IoT is the first decentralized relay architecture designed for IoT remote accessing and botnet malware prevention.
	
	\item We design smart contracts based relay billing scheme for fair relay service trading. The guaranteed remuneration motivates third-party relay providers to join for profit. The designed relay protocol solves possible disputations by making use of the objective and deterministic smart contract code execution. 
	
	\item Precautionary defense against future unknown malware is achieved by utilizing misbehavior reporting scheme and the concept of N-version programming\cite{chen1995n}. Thanks to the diversity of software implementations,  a given exploit can only work on a portion of the connected devices. Once the exploit fails on \emph{any} IoT device, the attacker's deposit would be confiscated. 
%since it is impossible for attackers to find any attack method with 100 percent success rate, attackers are frustrated by the risk of losing deposit cryptocurrency.  
	
%	\item We propose the idea of utilizing forensic records of unsuccessful attacking attempts to punish attackers and realize it via blockchain smart contracts. In this way,  attackers' intention of performing botnet scanning attacks is deterred due to the fear of losing cryptocurrency deposits. 
	
	\item We evaluate the overhead of the executing smart contract codes on Ethereum testnet and show that the solution is practical with acceptable cost.
\end{itemize}




Conventional centralized communication models having all devices connected to a central cloud server make the cloud server become the bottleneck and target of attacking~\cite{liang2017towards}.

Ideally, we would be able to patch all vulnerable IoT devices, but given the diversity of equipment, architecture, and attacks, this is extremely challenging





%  The fairness of service trading is justified by smart contract code, with which misbehavior of sending malicious attacking packets can be reported for punishment.  Also, misbehavior servers would be reported and eliminated from the relay sharing network, and relay service users can always switch to secure relay server as replacement of components. In this way, an indirect security patch method is achieved to defeat future unknown IoT malware.





% Different from previous work on IoT malware defense, our work has following advantages:
% \begin{enumerate}
%     \item Our work provides precautionary defense to defeat unknown malware attack in the future. The work aims to block all unauthorized traffic from attackers, instead of ex-post countermeasure like honeypot or IDS.
%     \item Our work requires no trusted third party or secure infrastructure. Our work proposes a self-governing system that requires no participation of any centralized agents or vendor.
%     \item Our work requires minimal assumption about the robustness of software. Our work only relies on the security of operating system kernel and all other software including the proposed handler itself can be assumed insecure.
%     \item Our work find ways of imposing risk of penalty on attackers' scanning behavior by leveraging smart contract and n-version programming.
% \end{enumerate}

%Our work seeks to find proactive way to defend future malware attacks. Like other traditional proactive defense mechanism, we utilize additional security software to achieve the goal. However, the difference is, in our work, we don't need to assume the added software is secure and trusted and we minimize the security assumption by assuming all applications except operating system kernel modules are possibly insecure. There will always be newly discovered security flaws and not reasonable to develop a perfect security software. So, rather than rely on the idealized security software to identify and reject attackers, we choose to find feasible way to punish attacking behaviours.

%In our work, we propose novel decentralized relay model for smart home IoT remote accessing. By eliminate the centralized relay server, security risk of single point failure is mitigated and vendor don't have to put into massive effort to protect the relay server against attackers.We also proposed innovative award and penalty system based on smart contract to incent third party individuals to join the relay network and deter the malicious participants.
%From some recent report <...TODO...> about the IoT botnets, we found except Mirai, nearly all successors are targeting on home routers. The reason is explicit: other IoT devices are usually hide behind the Network Address Translation (NAT) which cannot be directly accessed from Internet, while home routers function as home gateway have public IP address to be scanned by botnet attackers.

% That means, NAT provides additional protection for IoT devices by make them inaccessible from proactive scanning. On the other hand, the potential of IoT botnet has not been fully released, infecting the devices behind the NAT may become the interests for future IoT botnet attackers. To make these IoT devices been accessed remotely, vendor operated cloud server are used as relay. In this scenario, IoT devices initiate connection to the public accessible cloud server during boot up procedure and maintain heartbeat session. In this way, remote controller can easily connect to the IoT device by initiating connection with the relay server. However, since all IoT devices from the same vendor are connected to the same cloud server, cloud server becomes the security bottleneck. Attackers can easily get the domain name and address of the cloud server by buying a real device. Once the cloud server is taken down, attackers can immediately get control of all connected devices that shares similar security flaws. As a result, attackers can infect all these devices in short time with very high scan hitting rate. Since attackers has pre-acquired knowledge about the victim devices, more dangerous attacks may be conducted by attackers.

%Cloud relay architecture also induce heavy burden for vendors. As we'll illustrated in section \ref{sec:vul_in_cloud}. Some low cost vendors just leaving the server running without any security mechanism and doing relay for any requesters without verifying their identity. Attackers can easily access the connected IoT devices with randomly generated device id, once the get response from device, attackers may brute-force crack the accessing password or take down the device by exploiting software vulnerabilities.


The rest part of the paper is organized as follows. In Section \ref{sec:background}, we present the  background. In Section \ref{sec:cur}, we discuss the weaknesses of the centralized IoT accessing model. In Section \ref{sec:design}, we propose our design of relay-sharing IoT accessing method. Section \ref{sec:pod} and Section \ref{sec:penalty} describe the details of fair relay work proof and punishment on misbehavior during relay, respectively. Security analysis and experiments are presented in Section \ref{sec:secanalysis} and Section \ref{sec:exp}, respectively. We present the related work in Section \ref{sec:relatedwork} and conclude in Section \ref{sec:con}.



	
	
	




